HappyRouting: Learning Emotion-Aware Route Trajectories for Scalable In-The-Wild Navigation

Routes represent an integral part of triggering emotions in drivers. Navigation systems allow users to choose a navigation strategy, such as the fastest or shortest route. However, they do not consider the driver's emotional well-being. We present HappyRouting, a novel navigation-based empathic car interface guiding drivers through real-world traffic while evoking positive emotions. We propose design considerations, derive a technical architecture, and implement a routing optimization framework. Our contribution is a machine learning-based generated emotion map layer, predicting emotions along routes based on static and dynamic contextual data. We evaluated HappyRouting in a real-world driving study (N=13), finding that happy routes increase subjectively perceived valence by 11% (p=.007). Although happy routes take 1.25 times longer on average, participants perceived the happy route as shorter, presenting an emotion-enhanced alternative to today's fastest routing mechanisms. We discuss how emotion-based routing can be integrated into navigation apps, promoting emotional well-being for mobility use.

==> rebuttal_letter_chi24.tex <==
We thank the reviewers for their valuable feedback. We address the points in the following.

NOVELTY [1AC, 2AC, R2, R3]
We thank the reviewers for the reference and clarifications regarding the novelty of our work. We included the work by Wang et al. and described the difference to our work in the introduction and related work section. The authors present a heuristic model that determines a route based on traffic and historical emotions of a previously driven route. While prior work has introduced the concept of identifying a "happy route" or an emotion-centric navigation system, a practical emotion-routing system has not been demonstrated nor evaluated in real-world situations on unseen routes, thus relying on heuristics for previously driven routes. We clarified the novelty in the related work section. We also added a table in Section 2.3 to summarize the differences between previous and our research. 

STUDY DESIGN CLARIFICATIONS & RESULTS [1AC, 2AC, R2, R3]
We thank the reviewers for suggesting more details regarding study design and statistical results. We added a paragraph at the end of Section 4.4 for more information on how the F1 score averages out over many predictions.

We added descriptions of the starting & end point in the in-the-wild study in Section 5.1. Previous work suggests that commuting is the most common trip type [1, 2]. The trip length was substantiated by a study identifying the global average trip duration of 15 minutes [3]. Vehicle usage and trip length vary heavily depending on country and other factors.

We acknowledge the small sample size limiting the generalizability towards cultural, diversity, and gender aspects. We believe though, that our study is an important first step towards real-world insights. As suggested by the reviewers, demographic limitations of the study and the small sample size were added as limitations in the discussion.  

We thank 1AC, R2, and R3 for suggesting how to improve the statistics. We updated the statistics in Section 5.1 ("Valence-Arousal-Dominance Analysis") by adding more details to the statistics and the effect size. We compared the valence, arousal, and dominance scores after the ride, where we did not find a statistically significant effect. The route order had no statistical impact on participant ratings. Seven participants began with the happy route.

SAMPLE & DATASET SPECIFICATION [1AC, R2, R3]
We have updated the datasets' description to include their acquisition details. Participants were recruited via a dedicated mailing list of colleagues interested in participating in research projects. They gave explicit consent to participate and signed a detailed informed consent form explaining the study's aims and rights. In addition, the research was ethically approved by an independent review board to ensure compliance with recognized ethical standards and procedures (Section 5.1). Generating the dataset is now documented in the appendix (see Section 'Description of the classifier dataset').

MISC [1AC, 2AC, R2, R3]
We have incorporated all writing suggestions. In addition, we have placed our results in the context of previous work, added a table in Section 2.3 to describe how our work differs from previous work, and compared our results to previous work in the discussion. We are happy that the reviewers recognize the need to discuss the adverse effects that HappyRouting may have. We have added paragraphs in Sections 3.3 and 7.3 to show how driving automation could be affected. We are compelled by the impact of physiological sensing (e.g., improved classification) and have added this to Section 7.5. 

We have clarified in the caption of Figure 1 and Section 5.1 that the routes shown are examplary and do not stand for the routes evaluated in the user study. We have renamed "pre-post" to "before-after". We agree with R3 that Section 4.1 reads like a list of system requirements and therefore renamed the section to "Requirements". R3 also asked for more information about the features (e.g., feeltemp & greenness). We added a reference explaining why we chose these features based on the work of Braun et al. [4] and how they were obtained. We agree with the citation of the FERPlus paper ([5] in the paper) and the dataset used ([8] in the paper). We clarified the difference in the description of the title of Table 3.

We have implemented all suggested changes and suggestions and are ready to provide the paper for the camera-ready deadline. Thank you very much for your detailed reviews! 

REFERENCES
[1]: de la Fuente Layos, L (2007). Passenger mobility in Europe (No. Catalogue Number: KS-SF-07-087-EN-N).
[2]: Ramos, É (2020). Understanding daily car use: Driving habits, motives, attitudes, and norms across trip purposes.
[3]: O'Riordan  (2022). How and why we travel–mobility demand and emissions from passenger transport.
[4]: Braun, M (2021). Affective automotive user interfaces–reviewing the state of driver affect research and emotion regulation in the car.

==> revisions_required.tex <==
done -> orcid authors included in pdf -> david
done -> remove bold table and figure labels -> luis
done -> metadata from acm copyright receipt -> david
done -> contact email adress -> david 
done -> convert to acmlarge -> david
include footer on all pages -> thomas
footnote not spread over two pages -> thomas
done -> Figure 6,7,8 remove Type 3 fonts -> Satiya (this is the most time-sensitive issue, let me know how I can help)
done-> Figure 10 remove Type 3 fonts -> David











1AC:   Dear authors, the reviewers have acknowledged the significant effort that has been put in this revision, especially in extending the dataset. After reading their    comments and reading the revised manuscript I am happy to recommend acceptance of this work provided that you address the comments of reviewers 2 and 4 in a minor revision. As usual, please provide a report explaining how you addressed each one.


2AC:   As a general and final comment I think the paper can be accepted but there are
    still some points to be improved (minor changes):
    - English revision of the text
    - Please check the results presented in Table 2 and 4 -> done (recall and standard deviations of UAR were wrongly calculated, put in new numbers in table)
    - Provide the link for the public dataset. -> done


R3: None

R4: 
    Thanks for the revision, where most of my previous comments were addressed. In the
    updated version, there is still something very unclear or inconsistent, which
    needs to be addressed further:

    - on line 534 said the collected data last 663 minutes, but then after data
    preprocessing on line 622, the remained data lasts 677 minutes... And again, the
    mean duration on line 534 is around 14 min, while in fig6 average is 11.5 min,
    then 11.5*48 should be 552 minutes in total? Then, on line 1216, "the average
    session duration is around 15 minutes". It is very confusing.
    -> done (changed the numbers accordingly)

    - Acc is exactly the same as (weighted average) recall in Tables 2 and 4, please
    remove one of them. -> removed recall in Table 2 and Table 4, made best numbers bold in Table 4

    - in table 4, it cannot be true to have precision equal to 1 everywhere for all
    classes. Something must be wrong. -> the recall and precision values were wrongly calculated. We removed the recall from the table and changed the precision features.

    - Please add confusion matrix of the best feature and all features just as in Fig
    10.

authorship sharing with Luis -> done



revisions text

Dear Editors, Dear Reviewers,

We thank you for the positive feedback regarding the latest major revisions. 

We made all minor revisions requested to address all comments raised by the reviewers.

Below, we provide a response to the minor reviews.

Yours sincerely,
 
The Authors


We put significant effort in revisioning the text with two native speakers and changed some wording in the manuscript. In particular, we improved the readability and comprehensiveness of the Introduction, Related Work, Method and Discussion section. We found that some parts of the text sounded repetitive and stripped the corresponding paragraphs.
We double checked the results presented in Table 2 and 4 and corrected the numbers (in detail see revisions of R4). 
The link for the public dataset is now in the paper and available to anyone (https://github.com/msatiya/unobtrusive_driver_emotion_ds/).
We thank the reviewer for pointing out the confusing data duration statistics. We double checked all numbers for consistency and revised the manuscript accordingly. We thank the reviewer for pointing this out. We found a summarizing error in the precision and recall metric. As recommended by the reviewer, we removed recall in Table 2 and Table 4 (unweighted average recall is still reported). Furthermore, we indicated best prediction numbers bold in Table 4 to make the table more readable. We added a confusion matrix of a Random Forest classifier using all features side-to-side to Fig. 10.  To improve readability and reduce paper length, we decided to move the confusion matrix to the Appendix.


==> sections/experiment.tex <==
Our study is divided into two parts. The first part of the study is a within-subject-design, in-the-wild study where participants are using \system{} navigating them either through the fastest or happiest route. Second, in a numerical analysis, where we compare randomly sampled start-end routing choices, we assess the properties of the routes recommended by \system{}.



\subsection{In-The-Wild Driving Study}
We conducted a blind, within-subject, in-the-wild study to evaluate the driving experience of \system. We recruited thirteen participants (eleven self-identified as male, two self-identified as female) with an average age of $27\pm (8.51)$ years. Six participants occasionally drive (i.e., less than 10,000 km/year), six participants drive moderate distances (i.e., between 10,000 and 20,000 km/year) and one participant is a frequent driver (>20,000 km/year). \textcolor{black}{The complete study took about an hour for an individual driver and we scheduled the participants on different days throughout the week leading to different weather and road conditions for the evaluation.}
%The study took place on seven days.

The participants accessed a vehicle with a \chreplaced[id=1AC]{standard Android}{normal android} smartphone attached to the windscreen (see Figure~\ref{fig:phone_placement}). We gave the participants time to get familiar with the car and explained that they can drive like they normally do (hearing music, etc.). \textcolor{black}{Although we let the people decide themselves how to drive, only one participant decided to listen to low-volume music while driving.\footnote{ Music has shown to be a factor influencing emotions while driving~\cite{van2012influence}. }} We asked the participant to use our \system{} app just like a \chreplaced[id=1AC]{an ordinary}{normal} navigation app. The start and end location was chosen to be in a 15 minute drive away with segments including rural and urban segments. The start and endpoint of the drive were kept consistent for all participants to ensure comparability. \textcolor{black}{Within the same route the static contextual elements such as road types \chreplaced[id=1AC]{have not changed}{are not changing} across participants, however, the \chreplaced[id=1AC]{dynamic}{fluid} properties such as traffic flow are varying factors for the emotion classification engine.}

We \chreplaced[id=1AC]{hid}{hide} the routing choice (fastest or happy routing) in the app from the user to ensure that there is no confirmation bias (i.e., blind route choice). Overall the one-way driving had a duration of approximately twelve minutes for the fastest route and 14 minutes for the happy route, depending on individual traffic conditions.

We \chreplaced[id=1AC]{collected}{collect} subjective data of the drivers after each ride. This means that the drivers \chreplaced[id=1AC]{had}{will have} the chance for a subjective assessment of a route and their corresponding emotions felt before and after the driving. 
Before and after driving, we \chreplaced[id=1AC]{assessed}{assess} the emotional state (valence, arousal) of the driver via a self-assessment manikin (SAM) framework~\cite{bradley1994measuring} using a five point Likert scale. \textcolor{black}{For reproducibility, we provide a full description of the questionnaire together with further study clarifications in the appendix.}

The outline of the study is presented in Figure~\ref{fig:experimental_study_design}. The navigation mode (i.e., happy or fastest) was left blind and was randomly chosen for the participant, so that they were not able to tell which navigation mode \chreplaced[id=1AC]{was active}{they were driving} (7 out of 13 participants drove the happy route first). 
\begin{figure}[h]
    \centering
    \includegraphics[width = 1\linewidth]{figures/experiment/ExperimentalStudy3.pdf}
    \caption{Experimental design of the in-the-wild emotional navigation study. The endpoint of the second drive was set to be the start point of the first drive.}
    \label{fig:experimental_study_design}
\end{figure}



\begin{figure}[h]
    \centering
    \includegraphics[width = 1\linewidth]{figures/experiment/phone_setup2.pdf}
    \caption{Implemented navigation app that supports normal and happy routing. The app is placed on the windshield and has the same functionality as normal navigation apps (turn-by-turn navigation, voice output for hinting next directions). }
    \label{fig:phone_placement}
\end{figure}

\subsection{Numerical Analysis of Routes} 
To offer a broad assessment of the recommended happy routes by our system, we \chreplaced[id=1AC]{performed}{perform} an offline numerical analysis. First, we \chreplaced[id=1AC]{downloaded and computed}{download and compute} the emotional prediction layer for a map of a medium-sized, polish city ($12$ km $ \times 12$ km). Then, we sample a large number of equally-distributed, random start and end points ($N=1000$) and search for the happy and fastest route. We then analyze the route trajectories segments by computing several characteristics: road types, greenness, traffic conditions, and curviness. We furthermore compute the travel time, distance, as well as the overlap of fastest and happy route.


%Before and after a route, we asked questions related to their emotional state. 

%We aim for a subjective assessment of the situation and the influence of the context on the user experience, as well as, the general user emotion. %Since the gathering of subjective during a real-world driving situation is crucial in terms of ethical safety considerations, we ask the driver the questions in Table \ref{tab:testing_questionaire} before and after the drive. 

%We describe the methodology of our approach in the following.

%Participants are asked to rate two routes regarding their emotional attractiveness to validate the feasibility of affective routing.
%\subsection{Web Survey}
%We conducted a web survey to collect subjective feedback about the feasibility of affective routing from drivers. 17 participants participated in the web survey. The participants were recruited through a company channel to assess the systems route recommendation. We used a map engine and showed two non-labeled routes to the user. The route was chosen to take approximately 20 minutes. We asked the participants to describe the route and provide an estimate which route they think is fastest and makes them the most happy. The survey was done in three parts including a piloting phase and subsequent twofold evaluation in two different cities. The pilot phase was conducted using two routes of the first city with four participants. After the evaluation of results and refinement of changes in the questions formatting, wording and clarification, the main study started. To simplify the process we have picked two cities where majority of participants lived and probed the participants if they already know the routes. Participants were presented with two routes, where in the first city the first route was the fastest route and the second route the route that should induce happiness. In the second city, the first route was the route inducing happiness and route two was the fastest.

% \begin{figure}[h]
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/route_1.png}
%         \caption{Route one was the fastest in the web survey.}
%         \label{fig:route_1_bialystok}
%     \end{minipage}%
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/route_2.png}
%         \caption{Route two was the happy route.}
%         \label{fig:route_1_bialystok}
%     \end{minipage}
% \end{figure}

% \begin{figure}[h]
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/Route 1.png}
%         \caption{Route one was the happy route.}
%         \label{fig:route_1_krakow}
%     \end{minipage}%
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/Route 2.png}
%         \caption{Route one was the fastest in the web survey.}
%         \label{fig:route_1_krakow}
%     \end{minipage}
% \end{figure}


% Justify the study design (why do we do a web survey and a in-the-wild study)

%\subsection{Aparatus and Method}

%\subsection{Method}



%\subsection{Procedure}

%We attached the participants with a vital-monitoring wearable (Empatica E4) to gather electrodermal activity, heart rate and skin temperature throughout the ride. Our system  requires to “wire up the driver” before the ride, however, we opted for not asking the drivers emotion within the ride for an unbiased driver experience.
%Nine participants (1 female) were invited through a mailing list to participate in the real-world driving experiment.

 %The mean duration of the rides is 16 minutes ( SD = 11, min=7, max=52). The road type changed on average 7.9 times per ride.

%\subsection{Participants}



%add statistics of the user

%pendler - selbes Ziel zur selben Zeit an unterschiedlichen Tagen
%wenige Personen aber lange damit fahren -> von 4 -5 Leuten alle Daten fragen (verschiedene Tage, davor und danach)
%alle 10-15 min fahren
%1 min pro Minute proben
%After-Driving Questionaire: Traffic Conditions
%ruhige Studienteilnehmer (pre-questionaire) und dann Empatica anschliessen

%intensity of emotion measuring, and why they feel it
%how are we measuring emotion intensity
%do not add beep -> distract people, illegal, vital sign results, 
%if I do driving study: ask every 3 min 












%\subsection{Participants}
%We invited x participants through a mailing list of colleagues willing to participate in a driving study. They were asked to download our app and were equipped with a smartphone retainer before the ride.  

%\subsection{Physiological sensing}As shown in literature, physiological data can inform about the driver’s workload or emotional response. Hence, one approach will be to anonymously collect such data while driving. Our system  requires to “wire up the driver” before the ride, however, we opted for not asking the drivers emotion within the ride for an unbiased driver experience. Therefore, we attach an Empatica E4 that senses electrodermal activity, heart rate, skin temperature and accelerometer information from the driver throughout the route. 


==> sections/results.tex <==
We analyze \system{}'s effect on driver experience by analyzing the properties of the recommended routes in a numerical analysis and present the in-the-wild driving study results using the implemented smartphone navigation app. % David: Can we explain why you have selected these specific analysis strategies? It is unclear to me why you have chosen to do a statistical analysis (of what?), roadtype analysis, time-divergence analysis and so on.



\subsection{Numerical Analysis}
On the basis of the explained experiment setting in Section~\ref{sec:experiments}, we present the results of the \chreplaced[id=1AC]{system's}{systems} recommended routes of $1000$ randomly start-end points.

\paragraph{Route Time Analysis}
%We analyzed the gap between the fastest routing and the happy routing. 
We anticipated that taking the happy route would increase the travel time. Figure~\ref{fig:divergence_travel_times_happy_route} shows the relationship of the navigation mode on travel times. In effect, happy routes take longer in most of the rides. Using linear regression, we \chreplaced[id=1AC]{found}{find} that a one-minute increase in fastest routing requires on average 1.25 minutes (75 sec.) more time to drive using happy routing. Approximately $9\%$ of the start-end coordinates \chreplaced[id=1AC]{resulted}{result} in a situation where the happy route is identical to the fastest route ($overlap = 100\%$). The time difference can be substantial in individual cases, therefore, we stress a transparent time forecast to the driver when recommending happy routes. Notice that we can adapt the time differences of happy routing by changing the factor $\lambda$ for considering emotional weights in the routing optimization (see appendix Figure~\ref{fig:lambda}). 

\begin{figure}[h]
    \centering
    \includegraphics[width = 1\linewidth]{figures/results/byalstok_lambda=20_scatter_duration_divergence.pdf}
    \caption{Scatterplot of drive duration of normal vs. happy routing. The points are mostly on the top-left of the equal-traveltime line, meaning that happy routing takes generally longer to drive. The fitted regression ($R^2=0.82$, $BIC=4715$) with a slope of $\beta_1 = 1.25$ ($p=.00$) means that a 1-minute increase in normal routing will take $1.25$ minutes ($75$ $sec.$) more time to drive using happy routing. %The size of the scatter points represents the overlap of happy and normal route segments of the route (bigger radius - bigger overlap).
    } %the overlap of 1 is only happening in 9% of the cases
    % using 1000 sampled start-destination samples
    \label{fig:divergence_travel_times_happy_route}
\end{figure}

%To validate that happy routing takes longer to drive i.e., has a smaller-equal relationship to fastest routing, we randomly sample $1000$ start and destinations tuples and compute the two routing trajectories and track their corresponding travel times.


%This overlaps with a qualitative analysis of Pfleging et al.~\cite{pfleging:experiencemaps} where most participants clearly stated that they would only use the experience route if they do not lose much time. David: Discuss this in the discussion 
%Aus Pfleging: "Nevertheless, most participants clearly stated that they would only use the experience route if they do not lose much time (e.g., the difference in time and distance are too small to be the decisive factor, P#60). \cite{pfleging:experiencemaps}" Mar 9, 2022 12:01 PM, 
%On average, the participants would allow an experience route to take 20.9 % longer with regard to+ time and fastest route (SD = 21.3%), respectively 25.7 % with regard to distance and shortest route (SD = 28.2%).Mar 9, 2022 12:02 PM

 
\paragraph{Road Characteristic Analysis}
%\paragraph{Post-Routing Analysis}
%We analyze the route's characteristics coming from our system's architecture. We thereby also compute a curviness score of the route. The curviness is computed by...
%We could not include curviness as a input feature to the emotion prediction classifier as we predict emotions based on singular geocoordinates, however, our curviness index requires several road segments.


We \chreplaced[id=1AC]{analyzed}{analyze} the recommended happy and fastest route for their road types\chadded[id=1AC]{, illustrated} in Figure~\ref{fig:numerical_routing_context}. As the drive-time normalized route duration is only normalized per individual route, the values of the bars do not add up to $100\%$. We tested whether the distribution of the different road characteristics are significantly different ($p<.05$) using a non-parametric Mann-Whitney U test. Compared to the fastest route, we find that happy routes consist of more road segments with a higher predicted happiness score, higher curviness, higher freeflow speed, and maximum speed. We expect that the happy routes have a higher assigned higher happiness score due to our optimization formula~\ref{eq:routing_opt}. The curviness is computed using weighted measure of length of curves, which depends on a radius of circumscribed circle  passes through all three  consecutive geocoordinates in the route. Given $a,b,c$ as the length of the three sides of a triangle, the radius of the circumcircle is given by the formula:
\begin{equation}
    r = \frac{abc}{\sqrt{(a+b+c)(b+c-a)(c+a-b)(a+b-c)}}
    \label{eq:routing_opt}
\end{equation}
Curvy roads tend to increase the driving enjoyment, but also inhibit driving accident risks~\cite{haynes2007district}. Unhindered traffic scenarios can be captured by our proxy variable freeflow speed, which is higher for happy routes, and increase driver well being~\cite{roidl2014emotional}. Furthermore, we detect that the satellite-image-derived greenness (known part of the HSV spectrum) is lower for happy routes than the fastest route. Finally, we find that on-average happy routing includes significantly more residential roads. Residential roads often have reduced traffic and may reduce driver's stress and a more happy emotional state. In contrast, the recommended fastest routes contain significantly more living street and primary road segments, which often require more driver attention. As stated before, these findings are made on the basis of a large sample size and do not represent an individual recommended route. 





\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width =1\linewidth]{figures/results/numerical_analysis_context.png}
  \caption{}
  \label{fig:numerical_context_characteristics_analysis}
\end{subfigure}%
\hfill
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width =1\linewidth]{figures/results/roadtype_analysis.pdf}
  \caption{}
  \label{fig:numerical_roadtype_analysis}
\end{subfigure}
\caption{Characteristics of happy route vs. fastest route. \textbf{(a)} Distribution of `happiness', `curvature', `greeness', `max\_speed' and `freeflow\_speed' for the two routing modes. \textbf{(b)} Analysis of roadtypes of happy routing vs. fastest routing. We assess the roadtype of every road segment (x-axis) and compute the drive-time normalized route duration (y-axis). }
\label{fig:numerical_routing_context}
\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.7\linewidth]{figures/results/numerical_analysis_context.png}
%     \caption{Characteristics of happy route vs. fastest route. }
%     \label{fig:numerical_context_characteristics_analysis}
% \end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width = 1\linewidth]{figures/mockups/characteristics-happy-routes.jpg}
%    \caption{Caption}
%    \label{fig:characteristics_happyroute}
%\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width = .8\linewidth]{figures/results/roadtype_analysis.png}
%     \caption{Analysis of roadtypes of happy routing vs. fastest routing. We assess the roadtype of every road segment (x-axis) and compute the drive-time normalized route duration (y-axis). As the drive-time normalized route duration is only normalized per individual route, the values of the bars do not add up to 100\%. }
%     \label{fig:numerical_roadtype_analysis}
% \end{figure}

%\todo[inline]{TG: Conduct a short investigation of computational complexity to update weights of 100 sqkm?}


%The results of this statistical analysis are presented in Figure~\cite{fig:characteristics_happyroute}. % David: Can we describe the results in the text by, for example, how much of the different characteristics affected the traveltime?

%\begin{figure}
%    \centering
%    \includegraphics[width = 1\linewidth]{figures/results/roadtype_analysis.pdf}
%    \caption{Analysis of road types (number of lanes, classified road type and maximum speed limit) of the two routing choices (happy vs. normal) with $y$-axis showing the percentage of travel time spent on the individual elements.} %
%    \label{fig:barplot_roadtypes}
%\end{figure}


%\begin{figure}[h]
%    \centering
%    \includegraphics[width = 1\linewidth]{figures/mockups/environmental-change.jpg}
%    \caption{Caption}
%    \label{fig:environment_change}
%\end{figure}


%\subsection{Web Survey Results}
%For both cities participants indicated that route generated by the ``fastest'' weighting algorithm is fast or faster than the happy route. For the second city there was indication on big traffic on both the ``fastest'' and ``happy'' route. The answers regarding ``happy'' route in both cities indicated that the route is going to elicit happy emotions. In the first city it was indicated, that the route goes through the city center, which at the same time makes it interesting and prone to big traffic, depending on time of day.

% \begin{figure}[h]
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/bstok.png}
%         \caption{Mostly used adjectives to describe both happy and fastest routes in Bialystok questionnaire.}
%         \label{fig:bstok_adj}
%     \end{minipage}%
%     \begin{minipage}{.5\textwidth}
%       \centering
%         \includegraphics[width = 1\linewidth]{figures/offline_experiment/krakow.png}
%         \caption{Mostly used adjectives to describe both happy and fastest routes in Krakow questionnaire.}
%         \label{fig:krakow_adj}
%     \end{minipage}
% \end{figure}

% In general all participants noticed significant difference between both routes and in most cases indicated in one or more answers, that route generated by the ``happy'' algorithm is more interesting or more happy to drive. Thanks to the selection of routes described before, the participants indicated that at least 50\% knew both routes very well, while only 35\% knew one of the routes partially.

% There were also three general aspects of the system which were part of questionnaire:

% 1) When the participant would use the feature while driving?
% The answers were mainly around situations like: vacation, happy time, good weather, sightseeing, driving with friends. In general participants would use the system when condition is associated with happiness. Two of participants also indicated, that being not in hurry would make him use the system more often.

% 2) What type of elements should happy route include?
% The mostly repeated answers are:
% \begin{enumerate}
%     \item road quality and road state
%     \item points of interest like museums, architecture, interesting scenery or monuments
%     \item greenness of the surroundings
%     \item easiness of driving
% \end{enumerate}







%3) What features car should have to be useful in pair with happy navigation?
%The mostly repeated answers are:
%\begin{enumerate}
%    \item panoramic roof
%    \item radio and relaxing music
%    \item sightseeing suggestions
%    \item sport features
%\end{enumerate}

%\paragraph{Navigation}



%in the survey as well as in the in-the-wild experiment responded, that they would likely use the system. 

%\begin{figure}[h]
%   \centering
%    \includegraphics[width = 0.4\linewidth]{figures/offline_experiment/how_often.png}
%    \caption{How often would you use the system question answers (higher number is better).}
%    \label{fig:how_often}
%\end{figure}

% web survey is there for the classification of routes and get the impression of a happy routing app

%TODO: Intention and anticipated result?
%TODO: Presentation of two routes known to the user (e.g. commuters) and probe the associations with the routes?l

\subsection{In-The-Wild Study Analysis}

\todo[inline]{T: We identify user needs from related work and our user study questionnaire aiming at personalization (upper limit for travel time, reweighing emotion map layers, feature penalties). We disentangle the relationship between travel duration and happiness by related work [41, A3] (1AC, R1, R2). We asked the participants about their travel time budget to drive the happy route in a questionnaire and included this in the design of our system (setting of $\lambda$). }}

We describe the analysis of the in-the-wild study in the following. %We analyze the differences between the fast and happy routes, influence of road characteristics, and difference of the valence as well as arousal before and after driving.


% Analysis of Russel's continuum before and after interaction
\paragraph{Valence-Arousal Analysis Before and After Driving}
%\todo{more detailed description of how this was measured}
Our in-the-wild driving experiment explores the real-world feasibility and driver experience using happy navigation. 
We present the before and after analysis of arousal and valence score in Figure~\ref{fig:valence_arousal_before_after_in_the_wild}, that we assessed via a SAM questionaire (see section~\ref{sec:experiments}). We \chreplaced[id=1AC]{found}{find} that people gave a higher valence score\chreplaced[id=1AC]{, i.e.,}{i.e.} positiveness after driving the happy route. The mean valence score of happy routing before driving \chreplaced[id=1AC]{was}{is} 4.15 and \chreplaced[id=1AC]{increased}{increases} to 4.62 after driving ($11\%$ valence score increase). Using a paired t-test, we \chreplaced[id=1AC]{found}{find} that the difference \chadded[id=1AC]{in} valence of the happy route before and after is highly significant ($p=.007$)\footnote{We checked the normal distribution of the samples via a non-parametric Mann-Whitney U test: $p=0.04$.}. Therefore in our in-the-wild study, we \chreplaced[id=1AC]{showed}{show} that our happy routing has a positive effect on subjective felt positive emotions. The difference of arousal when driving happy route ($p= 0.111$) is not significant. Some participants felt calmer, whereas others were more excited after driving the happy route resulting in much larger variations in the arousal scores. The high variability likely \chreplaced[id=1AC]{originates}{comes} from the overall excitement of driving itself, which is highly person-related. While many empathic car applications envision to optimize arousal levels for safety reasons, we \chreplaced[id=1AC]{did}{do} not detect a significant change in arousal values in the wild. This finding contrasts common empathic car application motivations, focusing predominantly on improving arousal levels. In addition, we did not find significant before-after differences in valence or arousal when driving the fastest route. %We also find a much larger variety of the effect on arousal from driving the happy route. 



%We find, that people responded that after driving the fastest route rated the navigation to be: "..." (P1),. In opposition to that 

\begin{figure}[h]
    \centering
    \includegraphics[width = 1\linewidth]{figures/results/in_the_wild_valence_arousal_aggregate.pdf}
    \caption{Before and after driving analysis of arousal and valence questionnaire answers of the in-the-wild study. The lines indicate the standard deviation (vertical) of the responses where the means are connected via the dashed line.}
    \label{fig:valence_arousal_before_after_in_the_wild}
\end{figure}




\paragraph{Happy Navigation Driving Behavior}
In our in-the-wild questionaire, we saw high variability when and how wanted to use happy navigation functionality. After the driving experiment, we asked the participants "If the happy route would be longer, how much time would you sacrifice to drive a happy routing (assuming 20 min. drive for fastest routing)?". 9/13 of participants answered with $3-5$ min., while 3/13 drivers would like to only spend $1-3$ min. drive more. One participant stated, that he would even spend more than $10$ min. additional drive time to drive the happy route. This finding overlaps with the web-survey of Pfleging et al.~\cite{pfleging:experiencemaps}, where participants would allow an experience route to take $20.9\%$ longer with regard to time and fastest route ($SD = 21.3\%$). After driving the two routes, we asked the participant, which route they find longest to drive. While the fastest route took on average 2 min. less time, 8/13 participants felt, that the happy route was shorter. Combined with our finding, that people felt a higher positive emotional state after driving the happy route, we observe that happy routing influences the drivers to perceive drive time as shorter. Furthermore, in our study many participants (P1, P2, P3, P4, P6, P7, P8, P9, P11, P12, P13) stated that they would use the app in their leisure time, when they do not have time pressure. Interestingly, many participants responded to use our navigation only on the weekend (P9, P10, P12), preferably in the summer (P1, P2, P3, P4, P9, P10, P12), and not at night when the driving scenery is not visible (P8, P13). P2 mentioned he would use happy routes ``if a traffic jam is occurring and he could take lesser crowded, and more relaxed and unknown routes''. %Furthermore 4 participants want to use happy navigation primarily in the summer (P1, P2, P3, P4), and 2 participants (P7, P8) would use it on the weekend only. 


\paragraph{System Acceptance}
%The reception of the system was also very positive and visible in answers to question "how often would you use the system".
When the participants were asked "How likely would you use this system?" on a scale from 1 (rather not) to 5 (very likely), 11/13 participants (in-the-wild study) gave 4 and 5 ratings. Overall, we observed high demand for happy navigation, as only two participants gave a score of 3 and 2, respectively.


The study participants further introduced ideas for pairing happy navigation with other further in-car technology. The most prominent responses were that many participants associate happiness with music while driving. Therefore, many suggestions were made regarding automatic music selection during driving to math the route, or the other way around - to select the route to match music better.


We also asked the participants in a free-response question, "Do you think there are any societal and ethical implications of this navigation functionality? And if yes, which one?". Many participants said they do not see any ethical or societal implications (P6, P7, P9, P11, P13). Participants also responded with higher energy consumption costs and a more environmentally harmful behavior when driving a happy route (P1, P3, P10). P10 stated, that she sees a problem when happy routing only recommend nice driving routes, that other less-happy predicted places get no visibility, and high predicted-routes get visited often, thereby enhancing a self-enforcing effect what people see.
%a driving a happy route may often take longer and is more environmentally harmful due to higher fuel consumption.
% \begin{figure}[h]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/results/valence_plot_in_the_wild_driving_aggregate.pdf}
%   \caption{Valence values before and after driving.}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/results/arousal_plot_in_the_wild_driving_aggregate.pdf}
%   \caption{Arousal values before and after driving.}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Before and after driving analysis of arousal and valence questionnaire answers of the in-the-wild study. The lines indicate the standard deviation (vertical) of the responses where the means are connected via the dashed line. }
% \label{fig:valence_arousal_before_after_in_the_wild}
% \end{figure}
%The valence/arousal values are gathered via the self-assessment manikin framework~\cite{bradley1994measuring} using a five point Likert scale.

==> tables/feature_set_tab.tex <==
\begin{table}[h]
    \renewcommand\arraystretch{1.25}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccccccccccc}
    \hline
    \diagbox{\textbf{Feature Set}}{\textbf{Feature Context}} & \textbf{Personal} & \textbf{\begin{tabular}[c]{@{}l@{}}Session\\Time\end{tabular}} & \textbf{Motion} & \textbf{GPS} & \textbf{\begin{tabular}[c]{@{}l@{}}Traffic\\Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Weather\\Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Road\\Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Facial\\Expression\end{tabular}} & \textbf{Audio} & \textbf{\begin{tabular}[c]{@{}l@{}}Visual Complexity\\ (Object Detection)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Visual Complexity\\ (Segmentation)\end{tabular}} \\
    \hline    
    \begin{tabular}[c]{@{}c@{}}Automotive-OEM Setting\\With High Privacy Protection\end{tabular} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} \\
    \hline
    \begin{tabular}[c]{@{}c@{}}Optional User Setting\\For Improved Accuracy\end{tabular} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} \\
    \hline
    \end{tabular}%
    }
    \caption{\label{tab:feature_set} \textbf{ Use-Case Specific Feature Sets.} Table showing different feature set recommended for specific use-cases.}
\end{table}

==> tables/results_table.tex <==
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out) }\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Participant-Independent/Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions ( Azure )} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & 1 & .48 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & 1 & .66 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & 1 & .63 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .56 & 1 & .56 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & 1 & .63 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & 1 & .61 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .4  & .53 & 1 & .53 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .64 & 1 & .64 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & 1 & .66 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{1} & \textbf{.68} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: Unshuffled, Participant-Independent, Participant-Dependent. Accuracy (Acc.), precision (Prec.), recall and  weighted $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}




%old table with 3 presented features
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .40  & .53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation, leave-one-road-segment-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}



%removed leave one road segment out
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}


%\begin{table}[t]
%    \renewcommand\arraystretch{1.5}
%    \resizebox{\textwidth}{!}{%
%    \begin{tabular}{l|cccc|cccc}
%    \toprule
%     &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%      \midrule
%    \textbf{Feature Group} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} \\
%      \midrule
%    \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%    \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%    \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%    \midrule
%    \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%    \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%    \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%    \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%    \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%    \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%    \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%    \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%    \bottomrule
%    \end{tabular}%
%    }
%     \caption{\textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
%     \label{tab:results}
%\end{table}


\begin{table}[h]
    \renewcommand\arraystretch{1.5}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccccc|ccccc}
    \toprule
                          & \multicolumn{5}{l|}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} & \multicolumn{5}{l}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ \midrule
    \textbf{Feature Group} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Recall} & \textbf{\changed{UAR}} &\textbf{$F_1$} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Recall} &  \textbf{\changed{UAR}} & \textbf{$F_1$} \\ \midrule
    \multicolumn{1}{l|}{\textit{Facial Expressions (FERPlus)}} & \changed{.43 $\pm$ .12} & \changed{.46 $\pm$  .13}& \changed{.43 $\pm$  .12} & \changed{.13 $\pm$ .03} & \changed{.41 $\pm$  .13} & .27 & .93 & .27 & & .31 \\
    \multicolumn{1}{l|}{\textit{Facial Expressions (Azure)}} & \changed{.55 $\pm$ .13} & \changed{.48 $\pm$  .15} & \changed{.55 $\pm$  .13} & \changed{.17 $\pm$ .03} & \changed{.47 $\pm$  .13} &  .48 & .41 & .54 & & .47 \\
    \multicolumn{1}{l|}{\textit{VEmotion (VE)}} & \changed{ .52 $\pm$ .16} & \changed{.38 $\pm$  .17} & \changed{.52 $\pm$  .16} & \changed{.26 $\pm$ .09}  & \changed{.42 $\pm$  .17} & .66 & .61 & .63 & & .66 \\ \midrule
    \multicolumn{1}{l|}{\textit{Visual Complexity Segmentation (VC-Seg.)}} & \changed{.54 $\pm$ .14} &\changed{.48 $\pm$  0.12} & \changed{.54 $\pm$  .14} & \changed{.18 $\pm$ .03} & \changed{.44 $\pm$  0.16} & .63 & .53 & .57 & & .63 \\
    \multicolumn{1}{l|}{\textit{Visual Complexity - Object Detection (VC-ObjD.)}} & \changed{.32 $\pm$ .13} & \changed{.32 $\pm$ .13} & \changed{.5 $\pm$  .11} & \changed{.09 $\pm$ .02}& \changed{.37 $\pm$  .13} & .55 & .48 & .46 & & .59 \\
    \multicolumn{1}{l|}{\textit{VC-Seg. + Audio}} & \changed{.55 $\pm$ .14} & \changed{.49 $\pm$  .09} & \changed{.55 $\pm$ .14} & \changed{.17 $\pm$ .03} & \changed{.44 $\pm$  .17} & .63 & .53 & .57 &  &.63 \\
    \multicolumn{1}{l|}{\textit{VC-ObjD. + Audio}} & \changed{.48 $\pm$ .12} & \changed{.5 $\pm$  .11} & \changed{.48 $\pm$  .12} & \changed{.12 $\pm$ .01}& \changed{.45 $\pm$  0.13} & .61 & .50 & .53 &  &.62 \\
    \multicolumn{1}{l|}{\textit{Audio only}} & \changed{.37 $\pm$ .06}  & \changed{.49 $\pm$  .1} & \changed{.37 $\pm$ .06} & \changed{.1 $\pm$ .01} & \changed{.4 $\pm$  .09} &.53 & .47 & .47 & &.58 \\
    \multicolumn{1}{l|}{\textit{Audiovisual (OjbD. + Seg. + Audio)}} & \changed{.56 $\pm$ .14}  & \changed{.48 $\pm$  .15} & \changed{.56 $\pm$  .14} & \changed{.19 $\pm$ 0.03} & \changed{.44 $\pm$  .17} & .65 & .54 & .59 &  &.64 \\
    \multicolumn{1}{l|}{\textit{Location-based only}} & \changed{.57 $\pm$ .16}  & \changed{.44 $\pm$ .19} & \changed{.57 $\pm$  .16}  & \changed{.29 $\pm$ .11} & \textbf{\changed{.46 $\pm$  .18}} & .66 & .62 & .64 & &.65 \\ 
    \multicolumn{1}{l|}{\textbf{All features}} & \textbf{\changed{.58 $\pm$ .15} }  & \textbf{\changed{.43 $\pm$  .17}} & \textbf{\changed{.58 $\pm$  .15}} & \changed{.29 $\pm$ .08} & \changed{.45 $\pm$  .17} & \textbf{.68} & \textbf{.63} & \textbf{.66} &  &\textbf{ .67} \\  \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
    \label{tab:results}
   \end{table}

==> tables/results_table_participant_dependentonly.tex <==
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out) }\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Participant-Independent/Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions ( Azure )} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & 1 & .48 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & 1 & .66 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & 1 & .63 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .56 & 1 & .56 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & 1 & .63 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & 1 & .61 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .4  & .53 & 1 & .53 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .64 & 1 & .64 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & 1 & .66 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{1} & \textbf{.68} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: Unshuffled, Participant-Independent, Participant-Dependent. Accuracy (Acc.), precision (Prec.), recall and  weighted $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}




%old table with 3 presented features
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .40  & .53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation, leave-one-road-segment-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}



%removed leave one road segment out
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}


%\begin{table}[t]
%    \renewcommand\arraystretch{1.5}
%    \resizebox{\textwidth}{!}{%
%    \begin{tabular}{l|cccc|cccc}
%    \toprule
%     &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%      \midrule
%    \textbf{Feature Group} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} \\
%      \midrule
%    \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%    \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%    \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%    \midrule
%    \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%    \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%    \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%    \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%    \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%    \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%    \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%    \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%    \bottomrule
%    \end{tabular}%
%    }
%     \caption{\textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
%     \label{tab:results}
%\end{table}


\begin{table}[h]
    \renewcommand\arraystretch{1.5}
    \centering
        \caption{Random Forest Evaluation Results. We report the averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy, class-weighted precision, unweighted average recall (UAR) and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
    \resizebox{1\textwidth}{!}{%
    \begin{tabular}{l|ccccc}
    \toprule
      & \multicolumn{4}{l}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{9.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ \midrule
   & \textbf{Accuracy} & \textbf{Precision}  &  \textbf{\changed{UAR}} & \textbf{$\boldsymbol{F}_1$} \\ \midrule
    \multicolumn{1}{l|}{\textit{Facial Expressions (FERPlus)}} &  .33 $\pm$ .0 &  \changed{.41 $\pm$ .09} & .23 $\pm$ .04 & .36 $\pm$ .09 \\
    \multicolumn{1}{l|}{\textit{Facial Expressions (Azure)}} &  .39 $\pm$ .04 &  \changed{.42 $\pm$ .04} & .27 $\pm$ .0 & .38 $\pm$ .03 \\
    \multicolumn{1}{l|}{\textit{VEmotion (VE)}} & .65 $\pm$ .04 &  \changed{.63 $\pm$ .04} & \changed{.59 $\pm$ .01} & .64 $\pm$ .03 \\ \midrule
    \multicolumn{1}{l|}{\textit{Visual Complexity Segmentation (VC-Seg.)}} & .6 $\pm$ .04 &  \changed{.50 $\pm$ .04} & \changed{.38 $\pm$ .01} & .62 $\pm$ .03 \\
    \multicolumn{1}{l|}{\textit{Visual Complexity - Object Detection (VC-ObjD.)}} & \changed{.51 $\pm$ .06} &  \changed{.51 $\pm$ .06} &  \changed{.27 $\pm$ .01} & \changed{.56 $\pm$ .03} \\
    \multicolumn{1}{l|}{\textit{VC-Seg. + Audio}} & .61 $\pm$ .04 &  \changed{.51 $\pm$ .04} & \changed{.39 $\pm$ .01} & .61 $\pm$ .03 \\
    \multicolumn{1}{l|}{\textit{VC-ObjD. + Audio}} & .58 $\pm$ .04  &  \changed{.42 $\pm$ .04} & \changed{.32 $\pm$ .01} & .61 $\pm$ .02 \\
    \multicolumn{1}{l|}{\textit{Audio only}} & .52 $\pm$ .02 &  \changed{.39 $\pm$ .02} & \changed{.28 $\pm$ .01} & .57 $\pm$ .02 \\
    
    \multicolumn{1}{l|}{\textit{Audiovisual (OjbD. + Seg. + Audio)}} & .62 $\pm$ .03 &  \changed{.52 $\pm$ .03} & \changed{.43 $\pm$ .01} & .62 $\pm$ .02 \\
    
    \multicolumn{1}{l|}{\textit{GPS-infered features only}} & .65 $\pm$ .04 &  \changed{.63 $\pm$ .04} & \changed{.57 $\pm$ .11} & .57 $\pm$ .01 \\ 
    \multicolumn{1}{l|}{\textbf{All features}} & \textbf{.66 $\pm$ .03} &  \textbf{\changed{.65 $\pm$ .03}} & \textbf{\changed{.6 $\pm$ .01}} & \textbf{.67 $\pm$ .03} \\  \bottomrule
    \end{tabular}%
    }
    \Description[andom Forest Evaluation Results on participant-dependent modeling cross-validation.]{Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy, class-weighted precision, unweighted average recall (UAR) and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold). Overall 'All features' perfoms best in all metrics outperforming all baselines.}
    \label{tab:results_participant_dependent}
   \end{table}
   %Table~\ref{tab:results_participant_dependent} shows the

==> tables/results_table_participant_indepententonly.tex <==
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out) }\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Participant-Independent/Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions ( Azure )} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & 1 & .48 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & 1 & .66 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & 1 & .63 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .56 & 1 & .56 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & 1 & .63 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & 1 & .61 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .4  & .53 & 1 & .53 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .64 & 1 & .64 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & 1 & .66 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{1} & \textbf{.68} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: Unshuffled, Participant-Independent, Participant-Dependent. Accuracy (Acc.), precision (Prec.), recall and  weighted $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}




%old table with 3 presented features
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|cccc}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\parbox{4.5cm}{Global (Leave-One-Road-Segment-Out)} }} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .42 & .40 & .42 & .39 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 & .54 & .44 & .54 & .46 & .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21  & .63 & .64 & .63 & .61 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .58  & .54 & .58  & .52 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .34  & .46 & .34  & .38 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .59  & .54 & .59  & .51 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .49  & .44 & .40  & .45 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 & .39 & .41 & .39 & .40  & .53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .60 & .55 & .6 & .51  & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .64 & .64 & .64 & .62 & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.66} & \textbf{.65} & \textbf{.66} & \textbf{.63} & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation, leave-one-road-segment-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}



%removed leave one road segment out
% \begin{table}[t]
%     \renewcommand\arraystretch{1.5}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc|}
%     \toprule
%      &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%       \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%       \midrule
%     \textbf{Feature Group} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{$F_1$} &
%       \textbf{Acc.} &
%       \textbf{Prec.} &
%       \textbf{Recall} &
%       \textbf{ $F_1$} \\
%       \midrule
%     \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%     \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%     \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%     \midrule
%     \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%     \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%     \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%     \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%     \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%     \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%     \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%     \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%      \caption{\label{tab:results} \textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
% \end{table}


%\begin{table}[t]
%    \renewcommand\arraystretch{1.5}
%    \resizebox{\textwidth}{!}{%
%    \begin{tabular}{l|cccc|cccc}
%    \toprule
%     &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}} &
%      \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{4.5cm}{Participant-Dependent (Leave-One-Road-Segment-Out)} \end{tabular}}} \\ 
%      \midrule
%    \textbf{Feature Group} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} &
%      \textbf{Acc.} &
%      \textbf{Prec.} &
%      \textbf{Recall} &
%      \textbf{$F_1$} \\
%      \midrule
%    \textit{Facial Expressions (FERPlus) } & .43 & .15 & .12 & .12 & .27 & .93 & .27 & .31 \\
%    \textit{Facial Expressions (Azure)} & .55 & .16 & .17 & .14 &  .48 & .41 & .54 & .47 \\
%    \textit{VEmotion (VE)} & .54 & .18 & .27 & .21 & .66 & .61 & .63 & .66 \\
%    \midrule
%    \textit{Visual Complexity Segmentation (VC-Seg.)} & .55 & .2 & .18 & .14 & .63 & .53 & .57 & .63 \\
%    \textit{Visual Complexity - Object Detection (VC-ObjD.)} & .33 & .14 & .11 & .11 & .55 & .48 & .46 & .59 \\
%    \textit{VC-Seg. + Audio} & .55 & .2 & .18 & .15 & .63 & .53 & .57 & .63 \\
%    \textit{VC-ObjD. + Audio} & .48 & .16 & .14 & .13 & .61 & .50 & .53 & .62 \\
%    \textit{Audio only} & .38  & .14 & .12 & .12 &.53 & .47 & .47 & .58 \\
%    \textit{Audiovisual (OjbD. + Seg. + Audio)} & .56  & .17 & .2 & .16 & .65 & .54 & .59 & .64 \\
%    \textit{Location-based only} & .58  & .19 & .28 & \textbf{.22} & .66 & .62 & .64 & .65 \\ 
%    \textit{All features} & \textbf{.59}  & \textbf{.21} & \textbf{.29} & .21 & \textbf{.68} & \textbf{.63} & \textbf{.66} & \textbf{ .67} \\ 
%    \bottomrule
%    \end{tabular}%
%    }
%     \caption{\textbf{Random Forest Evaluation Results.} Table showing averaged evaluation results for each of the feature groups across all evaluation steps: global classifier learning leave-one-participant-out evaluation and learning participant-dependent models. Accuracy (Acc.), class-weighted precision (Prec.), recall and $F_1$ scores. Values are averages from the 10-fold cross-validation (best values are indicated in bold).}
%     \label{tab:results}
%\end{table}


\begin{table}[]
    \renewcommand\arraystretch{1.5}
    \centering
        \caption{Random Forest Evaluation Results. Table~\ref{tab:results} shows averaged evaluation results for each of the feature groups in a global classifier learning leave-one-participant-out evaluation. We compute accuracy (Acc.), class-weighted precision (Prec.), unweighted average recall (UAR) and $F_1$ scores. Best values are indicated in bold.
    %Values are averages of the \changed{\nparticipants}-fold cross-validation (best values are indicated in bold).
    }
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
                          & \multicolumn{4}{l}{\textbf{\begin{tabular}[c]{@{}c@{}} \parbox{8.5cm}{Global (Leave-One-Participant-Out)}\end{tabular}}}\\ \midrule
    \textbf{Feature Group} & \textbf{Accuracy} & \textbf{Precision} & \textbf{UAR} &\textbf{$\boldsymbol{F}_1$} \\ \midrule
    \multicolumn{1}{l|}{\textit{Facial Expressions (FERPlus)}} & \changed{.43 $\pm$ .12} & \changed{.46 $\pm$  .13} & \changed{.13 $\pm$ .03} & \changed{.41 $\pm$  .13}\\
    \multicolumn{1}{l|}{\textit{Facial Expressions (Azure)}} & \changed{.55 $\pm$ .13} & \changed{.48 $\pm$  .15}  & \changed{.17 $\pm$ .03} & \changed{.47 $\pm$  .13}\\
    \multicolumn{1}{l|}{\textit{VEmotion (VE)}} & \changed{ .52 $\pm$ .16} & \changed{.38 $\pm$  .17} & \changed{.26 $\pm$ .09}  & \changed{.42 $\pm$  .17} \\ \midrule
    \multicolumn{1}{l|}{\textit{Visual Complexity Segmentation (VC-Seg.)}} & \changed{.54 $\pm$ .14} &\changed{.48 $\pm$  0.12} &  \changed{.18 $\pm$ .03} & \changed{.44 $\pm$  0.16} \\
    \multicolumn{1}{l|}{\textit{Visual Complexity - Object Detection (VC-ObjD.)}} & \changed{.50 $\pm$ .11} & \changed{.32 $\pm$ .13} &  \changed{.09 $\pm$ .02}& \changed{.37 $\pm$  .13} \\
    \multicolumn{1}{l|}{\textit{VC-Seg. + Audio}} & \changed{.55 $\pm$ .14} & \changed{.49 $\pm$  .09} & \changed{.17 $\pm$ .03} & \changed{.44 $\pm$  .17}  \\
    \multicolumn{1}{l|}{\textit{VC-ObjD. + Audio}} & \changed{.48 $\pm$ .12} & \changed{ \textbf{.50 $\pm$  .11}} & \changed{.12 $\pm$ .01}& \changed{.45 $\pm$  0.13} \\
    \multicolumn{1}{l|}{\textit{Audio only}} & \changed{.37 $\pm$ .06}  & \changed{.49 $\pm$  .1}  & \changed{.10 $\pm$ .01} & \changed{.40 $\pm$  .09} \\
    \multicolumn{1}{l|}{\textit{Audiovisual (OjbD. + Seg. + Audio)}} & \changed{.56 $\pm$ .14}  & \changed{.48 $\pm$  .15}  & \changed{.19 $\pm$ .03} & \changed{.44 $\pm$  .17} \\
    \multicolumn{1}{l|}{\textit{ GPS-infered features only }} & \changed{.57 $\pm$ .16}  & \changed{.44 $\pm$ .19} &  \changed{.29 $\pm$ .11} & \textbf{\changed{.46 $\pm$  .18}} \\ 
    \multicolumn{1}{l|}{\textbf{All features}} & \textbf{\changed{.59 $\pm$ .15} }  & \changed{.43 $\pm$  .17} & \textbf{\changed{.29 $\pm$ .08}} & \changed{.45 $\pm$  .17}  \\ 
    \hline
    \multicolumn{1}{l|}{\textit{Neural Network (All features)}} & \changed{.43 $\pm$ .14}  & \changed{.52 $\pm$  .15}  & \changed{.18 $\pm$ .06} & \changed{.43 $\pm$  .14} \\

    \bottomrule
    \end{tabular}%
    }
    \Description[Random Forest Evaluation Results]{The table shows averaged evaluation results for each of the feature groups in a global classifier learning leave-one-participant-out evaluation. We compute accuracy (Acc.), class-weighted precision (Prec.), unweighted average recall (UAR) and $F_1$ scores. Overall All features performs the best using a Random Forest classifier.}
    \label{tab:results}
   \end{table}


   %neutral only prediction results
%accuracy: 0.5688 +/- 0.203
%precision: 0.3648 +/- 0.2227
%recall: 0.5688 +/- 0.203
%uar: 0.3259 +/- 0.104
%f1: 0.4363 +/- 0.2254

==> tables/table_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\renewcommand\arraystretch{0.74}
    \resizebox{\textwidth}{!}{%
        % \begin{tabular}{|p{6cm}|p{1cm}|p{14cm}|}%{lll}
        \begin{tabular}[t]{>{\raggedright}p{0.3\linewidth}>{\raggedright}p{0.3\linewidth}>{\raggedright\arraybackslash}p{0.7\linewidth}}
        \toprule
        \textbf{Context}                    & \textbf{Feature}          & \textbf{Details}   \\
        \midrule
Reference Data                      & frame\_number             & The number reference for the session snapshot frame pair.      \\
                                    & timestamp                 & e.g. 21/10/15, 18: 55:39:0025                                  \\
                                    & audio\_file\_path         & p\_01/session\_id/audio.mp4                                    \\
                                    & front\_frame\_path        & p\_01/session\_id/imgs/front\_frame\_501.jpg                   \\
                                    & back\_frame\_path         & p\_01/session\_id/imgs/back\_frame\_501.jpg                    \\
\midrule
Personal                            & sex                       & male, female, other                                            \\
                                    & car\_model                & e.g. VW Polo, Porsche Taycan                                   \\
                                    & age                       & Participant's age.                                             \\
                                    & participant\_id           & e.g. p\_01, p\_02                                              \\
                                    & emotion\_before           & Emotion before ride.                                           \\
\midrule
Session           & session\_id               & e.g. 0751B8E9-3357-47E3-A862-CBFC60B88555                      \\
                                    & session\_start            & e.g. 21/10/15, 18: 54:49:0015                                  \\
                                    & session\_end              & eg. 21/10/15, 19: 14:69:0485                               \\
\midrule
Session Time       & weekday                   & Mon. Tue. Wed., Thurs. Fri., Sat., Sun.                        \\
                                    & daytime                   & Morning, Afternoon, Evening, Night.                            \\
\midrule
Motion             & acceleration\_x           & Acceleration on the x axis.                                    \\
                                    & acceleration\_y           & Acceleration on the y axis.                                    \\
                                    & acceleration\_z           & Acceleration on the z axis.                                    \\
                                    & vemotion\_acceleration  & (or acceleration\_v1) Acceleration as in VEmotion~\cite{bethge_vemotion_2021}.  \\

\midrule
GPS                & speed                     & Vehicle speed in km/h.                                         \\
                                    & latitude                  & Latitude value of current location.                            \\
                                    & longitude                 & Longitude value of current location.                           \\
\midrule
Traffic Data       & current\_travel\_time     & Current travel time in seconds.                                \\
                                    & free\_flow\_speed         & The free flow speed expected under ideal conditions.           \\
                                    & current\_speed            & The current average speed at the selected point.               \\
                                    & free\_flow\_travel\_time  & The travel time in seconds under ideal free flow conditions.   \\
                                     & reduced\_speed  & Calculated with \textit{free\_flow\_speed} minus \textit{current\_speed}.   \\
                                    
                                    
\midrule                           
Weather Data       & wind\_speed               & Outside wind speed in km/h.                                    \\
                                    & precipitation\_24h\_mm    & Rain fall measurement in millimetres.                          \\
                                    & feel\_temp\_outside       & "Feels like" temperature in Celsius.                           \\
                                    & cloud\_cover              & Percent representing cloud cover.                              \\
                                    & weather\_term             & e.g. cloudy, mostly cloudy, mostly sunny, sunny                \\
                                    
\midrule                               
Road Data          & road\_type                & e.g. cycleway, footway, living\_street, motorway, residential. \\
                                    & max\_speed                & Maximum allowed speed for the current road.                    \\
                                    & num\_lanes                & Count of available lanes on the road.                          \\

\midrule
Facial Expression Pred.             & facial\_expression\_label & Front-facing camera’s classified emotion|.                     \\

\midrule
Perceived Emotion                   & label                     & Emotion expressed by the participant during the experiment.    \\

\midrule                               
Audio          & audio\_amplitude  & Audio amplitude averaged for duration of correspondent chunk.  \\
                    & audio\_loudness                & Audio recording average loudness for duration of correspondent chunk.                  \\ 
                    & audio\_zero\_crossings & Audio zero crossing rate of correspondent chunk.\\ 
                    
                   

\midrule
Visual Complexity (Object Detection)

& num\_cars, num\_people, bycicles, pedestrians,  motorcycles, buses,  trucks, traffic\_lights, traffic\_signs 
& Num. of objects detected in the back-facing camera frame per class.       \\
                                   
                            
                                    & num\_med\_close\_objs, num\_very\_close\_objs, 
                                     num\_close\_objs, num\_very\_far\_objs,  num\_far\_objs
                                    
                                    
                                    & Num. of objects at an estimated distance from camera.   \\
                                    % & num\_very\_close\_objs    & Num. of objects at very close distance.                        \\
                                    % & num\_close\_objs          & Num. of objects at close distance.                             \\
                                    % & num\_very\_far\_objs      & Num. of objects at very far distance.                          \\
                                    % & num\_far\_objs            & Num. of objects at far distance. \\
\midrule
Visual Complexity (Segmentation) & road, sidewalk, building, wall, fence, pole, traffic light, traffic sign, vegetation, terrain, sky, person, rider, car, truck, bus, train, motorcycle, bicycle

& Percentage pixels in back-facing frame representing class. \\

                            
                         
                             
                       
\bottomrule
\end{tabular}%
}
\caption{List of all available features in the dataset. We group the features by context and provide exemplary values or a description in the details column. The columns `frame\_number', `timestamp', `audio\_file\_path', `front\_file\_path', `latitude' and `longitude' are not used as input for the machine learning models. }
 \label{tab:feature-list}
\end{table}

==> tables/tradeoff_table.tex <==
\begin{table}[H]
    \renewcommand\arraystretch{1.25}
    \centering
        \caption{Trading off ubiquitous feature stream importance. We show different cost computational and privacy eroding factors of features while trading them off against their influence on performance in the form of $F_1$ decrease.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll|cccc|cccc|c}
    \toprule
                     &                  & \multicolumn{4}{c|}{\textbf{Feature Acquisition Factors}}                                                                                             & \multicolumn{4}{c|}{\textbf{Privacy Factors}}                                                                                                                                                                                                                                                                                                                          & \textbf{Prediction Importance}                                              \\
    \midrule
    \textbf{Context} & \textbf{Feature} & \textbf{\begin{tabular}[c]{@{}c@{}}Required\\ Sensors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Complex\\ Preprocessing\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Locally\\ Computable\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Third-Party\\ API Dependent\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Transfer of User Data\\ over the Internet\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Personal\\ Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Sensitive\\ Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-Cabin\\ Recording\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$F_1$\\ Decrease\end{tabular}} \\
    \midrule
    Personal & \begin{tabular}[c]{@{}l@{}}\textit{sex} \\ \textit{car\char`_model} \\ \textit{age} \\ \textit{before\char`_emotion} \end{tabular} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}} 0.0 \\ 0.0 \\ 0.001 \\ 0.003 \end{tabular} \\
             %& \textit{car\char`_model}      & \text{\ding{51}} & \text{\ding{55}} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
             %& \textit{age}                  & \text{\ding{51}} & \text{\ding{55}} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.001 \\
             %& \textit{before\char`_emotion} & \text{\ding{51}} & \text{\ding{55}} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.003\\
    \midrule
    Session Time & \begin{tabular}[c]{@{}l@{}}\textit{weekday} \\ \textit{daytime} \end{tabular} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.0 \\ 0.001 \end{tabular} \\
                 %& \textit{daytime} & \text{\ding{51}} & \text{\ding{55}} & \textit{--} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.001 \\
    \midrule
    Motion & \begin{tabular}[c]{@{}l@{}}\textit{acceleration\char`_x} \\ \textit{acceleration\char`_y} \\ \textit{acceleration\char`_z} \\ \textit{vemotion\char`_acceleration} \end{tabular} & \textit{Accelerometer} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.002 \\ 0.005 \\ 0.001 \\ 0.0 \end{tabular} \\
           %& \textit{acceleration\char`_y}        & \text{\ding{51}} & \text{\ding{55}} & \textit{Accelerometer} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.005 \\
           %& \textit{acceleration\char`_z}        & \text{\ding{51}} & \text{\ding{55}} & \textit{Accelerometer} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.001 \\
           %& \textit{vemotion\char`_acceleration} & \text{\ding{51}} & \text{\ding{55}} & \textit{Accelerometer} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
    \midrule
    GPS & \begin{tabular}[c]{@{}l@{}}\textit{speed} \\ \textit{latitude} \\ \textit{longitude} \end{tabular} & \textit{GPS} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.025 \\ \textit{--} \\ \textit{--} \end{tabular} \\
        %& \textit{latitude} & \text{\ding{51}}  & \text{\ding{55}} & \textit{GPS} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \textit{--} \\
        %& \textit{longitude} & \text{\ding{51}} & \text{\ding{55}} & \textit{GPS} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \textit{--} \\
    \midrule
    Traffic Data & \begin{tabular}[c]{@{}l@{}}\textit{current\char`_travel\char`_time}  \\ \textit{free\char`_flow\char`_travel\char`_time} \\ \textit{current\char`_traffic\char`_speed} \\ \textit{free\char`_flow\char`_speed} \\ \textit{reduced\char`_speed} \end{tabular} & \textit{GPS} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.0 \\ 0.0 \\ 0.001 \\ 0.008 \\ 0.0 \end{tabular} \\
                 %& \textit{free\char`_flow\char`_travel\char`_time} & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
                 %& \textit{current\char`_traffic\char`_speed}       & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.001 \\
                 %& \textit{free\char`_flow\char`_speed}             & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.008 \\
                 %& \textit{reduced\char`_speed}                     & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
    \midrule
    Weather Data & \begin{tabular}[c]{@{}l@{}}\textit{wind\char`_speed} \\ \textit{precipitation\char`_24\char`_hours\char`_mm} \\ \textit{feel\char`_temp\char`_outside} \\ \textit{cloud\char`_cover} \\ \textit{weather\char`_term} \end{tabular} & \textit{GPS} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.001 \\ 0.0 \\ 0.009 \\ 0.001 \\ 0.0 \end{tabular} \\
                 %& \textit{precipitation\char`_24\char`_hours\char`_mm} & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
                 %& \textit{feel\char`_temp\char`_outside}               & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.009 \\
                 %& \textit{cloud\char`_cover}                           & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.001 \\
                 %& \textit{weather\char`_term}                          & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.0 \\
    \midrule
    Road Data & \begin{tabular}[c]{@{}l@{}}\textit{road\char`_type} \\ \textit{max\char`_speed} \\ \textit{num\char`_lanes} \end{tabular} & \textit{GPS} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.006 \\ 0.002 \\ 0.011 \end{tabular} \\
              %& \textit{max\char`_speed} & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.002 \\
              %& \textit{num\char`_lanes} & \text{\ding{55}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & 0.011 \\
    \midrule
    Facial Expression Pred. & \textit{facial\char`_expression\char`_label} & \textit{In-Cabin Camera} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \textit{--} \\
    \midrule
    Audio & \begin{tabular}[c]{@{}l@{}}\textit{audio\char`_amplitude} \\ \textit{audio\char`_loudness}\end{tabular} & \textit{In-Cabin Microphone} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \begin{tabular}[c]{@{}c@{}}0.001 \\ 0.001 \end{tabular} \\
          %& \textit{audio\char`_loudness}  & \text{\ding{51}} & \text{\ding{55}} & \textit{In-Cabin Microphone} & \text{\ding{55}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.001 \\
    \midrule
    \begin{tabular}[c]{@{}l@{}}Visual Complexity\\ (Object Detection)\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}} buses, bicycles, cars, close\char`_objs,\\
                                                                               far\char`_objs, med\char`_close\char`_objs,\\
                                                                               motorcycles, people, trucks, stop\char`_signs,\\
                                                                               traffic\char`_ligts, very\char`_far\char`_objs,\\
                                                                               very\char`_close\char`_objs \end{tabular}} & \textit{Outside-View Camera} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.0, 0.0, 0.0, 0.0\\0.0, 0.0\\0.0, 0.0, 0.0, 0.0\\0.0, 0.0\\0.001\end{tabular} \\
                                                                               %& \textit{num\char`_bicycles} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_cars} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_close\char`_objs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_far\char`_objs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_med\char`_close\char`_objs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_motorcycles} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_people} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_stop\char`_signs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_traffic\char`_ligts} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_trucks} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_very\char`_close\char`_objs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{num\char`_very\char`_far\char`_objs} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.001 \\
    \midrule
    \begin{tabular}[c]{@{}l@{}}Visual Complexity\\ (Segmentation)\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}} bicycle, building, bus, car, fence, \\
                                                                           motorcycle, person, pole, terrain, \\
                                                                           rider, road, sidewalk, vegetation, \\
                                                                           sky, traffic\char`_light, truck, \\
                                                                           traffic\char`_sign, wall\end{tabular}} & \textit{Outside-View Camera} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \text{\ding{55}} & \begin{tabular}[c]{@{}c@{}}0.0, 0.005, 0.0, 0.001, 0.0,\\0.0, 0.0, 0.0, 0.0,\\0.001, 0.0, 0.009, 0.001,\\0.0, 0.0, 0.0,\\0.002, 0.0\end{tabular} \\
                                                                           %& \textit{segment\char`_building} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.005 \\
                      %& \textit{segment\char`_bus} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_car} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.001 \\
                      %& \textit{segment\char`_fence} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_motorcycle} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_person} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_pole} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_rider} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_road} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.001 \\
                      %& \textit{segment\char`_sidewalk} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_sky} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.009 \\
                      %& \textit{segment\char`_terrain} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.001 \\
                      %& \textit{segment\char`_traffic\char`_light} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_traffic\char`_sign} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_truck} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
                      %& \textit{segment\char`_vegetation} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.002 \\
                      %& \textit{segment\char`_wall} & \text{\ding{51}} & \text{\ding{51}} & \textit{GPS} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & \text{\ding{51}} & 0.0 \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:tradeoff}
    \Description[Table showing a trade-off of feature streams. ]{Table showing a trade-off of feature streams. We report computation cost factors (required sensors, complex preprocessing, locally computable, third-party API dependency),  privacy eroding factors (transfer of user data over the Internet, personal data,  sensitive data, in-cabin recording) and the related feature importance.}
\end{table}

==> todo.tex <==
Todo:
based on IMWUT and CHI reviews



8) Limitations: There is no emotion-adaptation in this system as the route is recommended and not adapted in real-time by analyzing e.g. the expression of the driver while driving the route? -> explain non-interactivity of the system as a advantage as this is not-privacy intrusive (Thomas) 


Already done
1) why include features such as weather as input when they do not change per route? -> add 1-2 sentences in method that these features give person-level insights on route choice preferences (David) -> done 
7) Why are these features selected? -> write 1 sentence in method, explain availability in-all-in the wild settings, available before routing and cite Vemotion (David) -> done
4) Why did you choose Rnaodm Forest classifier? -> good performance, cite Vemotion and IMWUT in method furthermore easily deployable in-car (David) -> done
3) Limitations of the comparison of routes as we considered only 13 participants on two routes. -> Add limitations: 'Further experiments with a larger variety of roads and routes under vastly different conditions are needed to produce necessary evidence of the proposed models abbility to find happy routes' (David) -> done
9) What is the influence of the specific features on the model, provide feature importance metrics of the Random Forest? -> put feature importance in appendix (David) -> done
5)  Fig. 2 and Fig.4 are far away from reference -> check (David) -> done (would not change it)

2) Why does our model need to predict 6 emotions when it only optimizes 'happiness'? -> add one sentence to method section, that our model can be simplified to a binary classification setting however, we wanted to make use of a broad emotion classifier ensuring adaptability for other use-cases where other emotion predictions are needed (Thomas)
